$O(a)$-improved QCD+QED Wilson Dirac operator on GPUs

Markov Chain Monte Carlo simulations of lattice Quantum Chromodynamics (QCD) are the only known tool to investigate non-perturbatively the theory of the strong interaction and are required to perform precision tests of the Standard Model of Particle Physics. As the Markov Chain is a serial process, the sole option for improving the sampling rate is accelerating each individual update step. Heterogeneous clusters of GPU-accelerated nodes offer large total memory bandwidth which can be used to speed-up our application, openQxD-1.1, which is dominated by inversions of the Dirac operator, a large sparse matrix. In this work we investigate offloading the inversion to GPU using the lattice-QCD library QUDA, and our early results demonstrate a significant potential speed-up in the time-to-solution for state-of-the-art problem sizes. Minimal extensions to the existing QUDA library are required for our specific physics programme while greatly enhancing the performance portability of our code and retaining the reliability and robustness of existing applications in openQxD-1.1. Our new interface will enable us to utilize pre-exascale infrastructure and reduce the systematic uncertainty in our physics predictions by incorporating the effects of quantum electromagnetism (QED) in our simulations.

==> __sections/01-intro.tex <==
% This allows for compiling the file separately:
% \documentclass[main.tex]{subfiles}

% \begin{document}

% \todo{TODO}:
% * advent of GPU based supercomputers, coming from the needs of ML
% * lattice is memory bandwidth bound, GPU have high throughput
% * many degrees of freedom fit well onto GPUs
% * self-inventing the wheel would be counter productive
% * QUDA powerful library on GPUs
% * C* boundaries and why they are important
% * QCD+QED and why it's important

The goal of lattice Quantum Chromodynamics (lattice QCD) is to numerically simulate the interactions of quarks and gluons on a finite and discrete Euclidean spacetime grid, enabling first-principles predictions of hadron properties. 

Computing hadronic observables to subpercent precision, as needed for example to interpret the most recent Muon g-2 measurements~\cite{Muong-2:2023cdq,Gerardin:2020gpp}, poses formidable challenges. It requires simulating four dynamical quark flavors, incorporating quantum electrodynamics (QED) effects, using fine lattice spacings for reasonable continuum extrapolation, using physical quark masses, and high statistics. Meeting these demands substantially increases computational requirements for generating Monte Carlo samples of gauge field configurations on large lattices.
% ~footnote{See, for example, Ref.~\cite{Gerardin:2020gpp} for a more detailed picture of the complexities involved in computing hadronic contributions to $(g-2)_\mu$ to subpercent precision using lattice QCD.}.

The growing adoption of GPU-accelerated supercomputing in major facilities, largely driven by machine learning needs, presents new opportunities for using GPUs for lattice QCD codes. As lattice simulations are constrained by memory bandwidth rather than floating point operations, the high-memory throughput of GPUs is expected to give a speed-up for calculations.

Our code, openQxD-1.1~\cite{openqxd}, extends the widely used openQCD-1.6 package~\cite{openqcd}, which supports the $O(a)$-improved Wilson fermion discretization (from now on, we will refer to these codebases simply as openQxD and openQCD, respectively). openQxD extends openQCD by allowing the simulation of QCD together with quantum electrodynamics (QED). This is accomplished through the use of C$^\star$ spatial boundary conditions \cite{Kronfeld1991}, which respect locality and Gauss's law at the same time reducing finite-size effects compared to periodic boundaries or other lattice QED formulations. These features make openQxD a versatile tool for achieving higher levels of precision. The codebase is designed for efficient parallel execution on CPU-based supercomputing architectures.

openQxD uses the Hybrid Monte Carlo algorithm for dynamical fermion lattice simulations, where the most time-consuming task is the repeated inversion of a large sparse operator to solve the Dirac equation. This Dirac operator, which connects nearest neighbor points on a 4D Euclidean spacetime lattice, has indices for Dirac spin, color charge, and space-time. By porting the Dirac solver to GPUs, the overall execution time of openQxD is expected to be significantly reduced.

Among the various possibilities for GPU-accelerating lattice QCD calculations, we choose to interface openQxD with the QUDA library~\cite{QUDApaper}, which provides optimized algorithms for NVIDIA and AMD GPUs, including an efficient iterative solver for the Dirac equation. 
We implement C$^\star$ boundary conditions and QED effects, as these are features that are particular to openQxD and do not yet exist in QUDA. In this way we combine openQxD's comprehensive physics toolset with QUDA's GPU-accelerated operations, thus enhancing openQxD simulations with GPU performance.

The remainder of this paper is structured as follows: \cref{sec:02-openqxd} introduces the openQxD codebase, while \cref{sec:03-quda} describes the QUDA library. 
\cref{sec:04-interface} details the process of interfacing the openQxD application with the QUDA library: it discusses the modifications to the memory layout of lattice fields, the implementation of $C^\star$ boundary conditions, and the extension of QUDA to handle QCD+QED simulations.
%\cref{sec:05-solver} describes the steps needed to call QUDA solvers from openQxD, that is initialization, parameter setup, error handling, and finalization. 
%\cref{building_openqxd_against_quda} explains how to build openQxD with QUDA. 
\cref{sec:07-performance} includes benchmark tests of CPU and GPU implementations of the Dirac operator and solvers. Finally, \cref{sec:08-outlook} proposes future optimizations and summarizes the achieved GPU acceleration.

% \end{document}



==> __sections/02-openqxd.tex <==
% This allows for compiling the file separately:
% \documentclass[main.tex]{subfiles}

% \begin{document}

\newcommand{\Dw}{{D_{\mathrm{w}}}}

The openQxD code~\cite{openqxd} is an extension of the state-of-the-art
lattice QCD Markov Chain Monte Carlo code
openQCD~\cite{openqcd,Luscher:2012av}, which is written in the C89 standard
with MPI parallelization with proven strong-scalability to hundreds of
CPU-based nodes and specific optimizations for x86 architectures.
Due to the extensive suite of legacy applications based on openQCD, as well as
its renowned stability and reproducibility, our goal is to accelerate the code
by offloading the solution of a large linear system of equations
$\Dw\psi=\eta$, defined by the Dirac operator $\Dw$, to the
device using the QUDA library.
The solution of this system for many right-hand sides is the most time
intensive kernel of the Monte Carlo algorithm, whose correctness can be
checked a posteriori, thereby allowing us to retain the functionality of
existing applications while interfacing only a minimal set of parameters.

%The Wilson-Clover Dirac operator $\Dw$ is a nearest-neighbour stencil operator
%acting on a linear space of quark (or spinor) fields defined on a regular 4D
%cubic lattice of $V_\mathrm{G}=N_0N_1N_2N_3$ sites, typically in the range $10^6-10^8$.
%Due to the nearest-neighbour coupling, a good parallelization is achieved by
%domain decomposition, where a contiguous local volume of size $V_\mathrm{L}=L_0L_1L_2L_3$,
%which divides the global problem size, is associated with a single computing
%unit.
%With accessible problem sizes, the Dirac operator is poorly conditioned and
%multi-grid preconditioning such as the inexact deflation \cite{Lüscher2007deflation} provided in openQCD
%or its QUDA equivalent is needed to speed up the convergence of the iterative
%solvers used.

The problem which we wish to offload is defined by the right-hand
side spinor $\eta$, which may be represented in different ways depending on 
conventions. These different conventions need to be mapped into each other in the interface.
Likewise, the couplings between the sites, which define the Dirac operator, are
parameterized by a set of so-called vector (or gauge) field variables $U_\mu$
for the four directions $\mu=0,1,2,3$, which need to be passed through the interface as well.
Although these fields are periodically updated along the Markov chain, in
the measurement part of the workflow they are kept fixed.
Finally, it is convenient to precompute the site-local coupling called the
clover-field which is a function of the gauge-field variables.
All these parameters are represented in openQCD by arrays of structs of length of
the local lattice volume.
%which are described as follows.

% The double precision spinor field is stored as an array of $V_\mathrm{L}$ \code{spinor\_dble} structs (\cref{lst:spinor}), the gauge field is stored as an array of $4V_\mathrm{L}$ \code{su3\_dble} structs (\cref{lst:gauge}), whereas the clover field is an array of $2V_\mathrm{L}$ \code{pauli\_dble} (\cref{lst:clover}).

%The gauge field is stored as an array of $4V_\mathrm{L}$ \code{su3\_dble} structs (\cref{lst:gauge}), which rely on \code{complex\_dble} structs (\cref{lst:complex_double}). The double precision spinor field is stored as an array of $V_\mathrm{L}$ \code{spinor\_dble} structs (\cref{lst:spinor}), while the clover field is an array of $2V_\mathrm{L}$ \code{pauli\_dble} (\cref{lst:clover}). 

% \begin{lstlisting}[language=C++, caption=The  complex double struct, label=lst:complex_double]
% typedef struct
% {
%    double re,im;
% } complex_dble;
% \end{lstlisting}

% \noindent
% \begin{minipage}{\linewidth}
% \begin{lstlisting}[language=C++, caption=The gauge field struct, label=lst:gauge]
% typedef struct
% {
%    complex_dble c11,c12,c13,c21,c22,c23,c31,c32,c33;
% } su3_dble;
% \end{lstlisting}
% \end{minipage}

% %\todo{Since the struct complex double is present in the spinor and gauge-field structs, I believe it is better for the listing to be split.}
% % typedef struct
% % {
% %    double re,im;
% % } complex_dble;
% \begin{lstlisting}[language=C++, caption=The spinor field struct, label=lst:spinor]
% typedef struct
% {
%    complex_dble c1,c2,c3;
% } su3_vector_dble;

% typedef struct
% {
%    su3_vector_dble c1,c2,c3,c4;
% } spinor_dble;
% \end{lstlisting}



% \begin{lstlisting}[language=C++, caption=The clover field struct, label=lst:clover]
% typedef struct
% {
%    double u[36];
% } pauli_dble;
% \end{lstlisting}

The spinor field has indices $(x, \alpha, a)$ ($a$ running fastest), where $x=(x_0,x_1,x_2,x_3)$ is the lattice index (a Euclidean 4-vector), $\alpha \in \{0,1,2,3\}$ is the spinor index and $a \in \{0,1,2\}$ is the color index.

The gauge field instead has indices $(x_{odd}, \pm \mu, a, b)$, where $x_{odd}$ is the lattice index (only odd points, $V_\mathrm{L}/2$ elements), $\mu \in \{\pm 0, \pm 1, \pm 2, \pm 3\}$ is the direction of the gauge link (in positive as well as negative direction, i.e., 8 possibilities) and $a,b$ parameterize the row and column of the $SU(3)$-valued gauge link (row-major). Thus openQxD stores the gauge links in all $8$ directions at odd lattice points in contrast with most other common conventions which store $4$ gauge links in positive directions for every lattice point.

Finally, the clover field has indices $(x, \pm, i)$, where $x$ is the lattice index, $\pm \in \{+, -\}$ denotes the chirality (i.e. the upper ($+$) or lower ($-$) $6 \times 6$-block of the $12 \times 12$ clover matrix) and $i \in \{0, \dots, 35\}$ the $36$ non-zero real numbers needed to parametrize a $6 \times 6$ Hermitian matrix.

In addition to these data structs, already defined in openQCD, the openQxD package --
which provides an extension to incorporate electromagnetic gauge fields --
requires new functionality such as C$^\star$ boundary conditions
and additional degrees of freedom: these are described in more detail in
\cref{sec:qcd+qed,sub:cstar} and respectively.

% \end{document}


==> __sections/03-quda.tex <==
% This allows for compiling the file separately:
% \documentclass[main.tex]{subfiles}

% \begin{document}

QUDA \cite{QUDApaper} is a library written in CUDA C++ that contains a suite of efficient kernels and solvers to implement lattice QCD simulations (the current release version 1.1.0 complies with the C++14 and 17 standards). It is thus natural that QCD fields are represented by objects, and the pointers to the fields' values are accessible via their objects.

% making use of the modern C++ standards, an  with  making use of the object paradigm and a high degree of abstraction.
% \todo{exact standard?: by checking the CMakeFiles, QUDA v.1.0 got C++11 or 14, in v.1.1.0 needs C++14 or 17 (ref: \code{https://github.com/search?q=repo\%3Alattice\%2Fquda+c\%2B\%2B17\&type=code}, and 
% }, 

A spinor field is represented by an instance of \code{ColorSpinorField}, a gauge field by \code{GaugeField} and a clover field as \code{CloverField}, all of which inherit from the \code{LatticeField} class. The different degrees of freedom are realised in the inheriting classes. The actual numbers are accessible via a pointer whose accessor is called \code{data()}.

QUDA is highly optimized to run on multiple GPUs, specifically on NVIDIA and AMD cards. In addition, it offers a multi-threading backend.

% \end{document}


==> __sections/04-interface.tex <==
% This allows for compiling the file separately:
% \documentclass[main.tex]{subfiles}

% \begin{document}

Linking openQxD against QUDA involves three major steps:
1) The memory layout of lattice fields is a fundamental difference between the two applications. We implement an interface that reorders the fields to agree with the different conventions.
2) QUDA does not support $C^\star$ boundary conditions, so we implement them in the QUDA library.
3) QUDA does not support simulating QCD+QED either. This feature involves modifying the Wilson-Dirac operator and the clover term.

\subsection{Field reordering}

In order to use QUDA's functionality within openQxD, one has to build QUDA as a library, include the main header file (\code{quda.h}) and link openQxD against it. 
As an example for a QUDA function, we consider inversions of the Dirac operator, whose API call signature looks as follows:

\begin{lstlisting}[language=C++]
void invertQuda(void *h_x, void *h_b, QudaInvertParam *param);
\end{lstlisting}

Here, \code{h\_x} and \code{h\_b} are void pointers pointing to the host spinor fields in openQxD order, i.e. base pointers to arrays of \code{spinor\_dble} structs. The \code{QudaInvertParam} struct parametrizes the solver (see \code{quda.h} and Ref.~\cite{QUDApaper} for details).


We implement the reordering in the following classes in QUDA \cite{QUDApaper}:
\begin{itemize}
  \item \code{OpenQCDOrder} in \code{include/gauge\_field\_order.h} for the gauge field.
  \item \code{OpenQCDDiracOrder} in \code{include/color\_spinor\_field\_order.h} for the spinor field.
  \item \code{OpenQCDOrder} in \code{include/clover\_field\_order.h} for the clover field.
\end{itemize}

All of the fields have the Euclidean space-time index in common, so we begin by discussing the order of the lattice sites in the following section.

\subsubsection{Space-time coordinates}

Denoting the rank-local lattice extent in direction $\mu=0,1,2,3$ by $L_\mu \in \mathbb{N}$, we can write the lattice coordinate as a 4-vector, $x = (x_0,x_1,x_2,x_3)$, where $x_\mu \in \{ 0, \dots, L_\mu -1 \}$. openQxD puts time coordinate first $x = (t, \vec{x})$, which we refer to as (txyz)-convention. From that we can create a lexicographical index
\begin{equation} \label{eq:lexi}
\Lambda(x, L) := L_3 L_2 L_1 x_0 + L_3 L_2 x_1 + L_3 x_2 + x_3.
\end{equation}
openQxD orders the indices in so called cache-blocks; a decomposition of the rank-local lattice into equal blocks of extent $B_\mu \in \mathbb{N}$ in direction $\mu$. Within a block, points are indexed lexicographically $\Lambda(b, B)$ as in \cref{eq:lexi}, but the $L_\mu$ replaced by $B_\mu$ and $x$ replaced by the block local Euclidean index $b$, such that $b_\mu = x_\mu \mod B_\mu \in \{ 0, \dots, B_\mu -1 \}$.  
Furthermore, the blocks themselves are indexed lexicographically within the rank-local lattice decomposition into blocks, i.e. $\Lambda(n, N_B)$, where we denote the number of blocks in direction $\mu$ as $N_{B,\mu} = L_\mu / B_\mu$, and the Euclidean index of the block as $n$, such that $n_\mu = \lfloor x_\mu / B_\mu \rfloor \in \{ 0, \dots, N_{B,i} -1 \}$.

In addition, openQxD employs even-odd ordering, that is all even-parity lattice points (those where the sum $\sum_{\mu=0}^3 x_\mu$ of the rank-local coordinate $x$ is even) come first followed by all odd-parity points.

Therefore, the total rank-local unique lattice index is
\begin{align} \label{eq:ipt}
\hat{x} &= \biggl \lfloor \frac{1}{2} \Big( V_B \Lambda(n, N_B) + \Lambda(b, B) \Big) \biggr \rfloor + P(x) \frac{V}{2},
\end{align}
where $V_B = B_0 B_1 B_2 B_3$ is the volume of a block, $P(x)=\tfrac{1}{2}(1-(-1)^{\sum_\mu x_\mu})$ gives the parity of index $x$, and $b$, $n$ are related to $x$ as described in the text above.
%(see \cref{fig:index} for an example).

% \begin{figure}
%   \centering
%   \includestandalone[width=0.4\linewidth]{img/index} %without .tex extension
%   % or use \input{mytikz}
%   \caption{2D example ($8 \times 8$ local lattice) of the rank-local unique lattice index in openQxD (in time first convention (txyz)). The blue rectangles denote cache blocks of size $4 \times 4$. Gray sites are odd, white sites are even lattice points.}
%   \label{fig:index}
% \end{figure}

This is implemented in openQxD by the mapping array \code{ipt}, $\hat{x} \coloneqq \text{ipt}\left[\Lambda(x,L)\right]$. Such mapping arrays are not recommended on GPUs due to shared memory contentions and memory usage. Instead, it is advisable to write a pure function $f \colon x \mapsto \hat{x}$ that implements \cref{eq:ipt} by calculating the index on the fly such that the compiler can properly inline the calculation.

We write the \code{OpenQCDDiracOrder} class that implements a \code{load()} and a \code{save()} method for the spinor fields. These two methods are called by QUDA in a loop with all possible values for \code{x\_cb} and \code{parity}, where \code{x\_cb} denotes the (local) checkerboard site index and \code{parity} the parity of the point. QUDA provides an (inlined) function \code{getCoords()} to translate the checkerboard and parity index into a (local) 4-vector $x = (\vec{x}, t)$ with time coordinate last ((xyzt)-convention). After permuting the coordinates into (txyz)-convention, we can query the mapping function $f$ to obtain for the desired lattice point the offset from the base pointer in openQxD and copy the data. That data might have additional indices that we describe in the
following.

\subsubsection{Spinor Field}

As mentioned previously, spinor fields have indices $(x,\alpha,a)$, where we describe how to transform the space-time index $x$ in the previous section. Both QUDA and openQxD use the same order for spinor index $\alpha$ and color index $a$. Thus at each space-time index we can copy $12=4 \cdot 3$ consecutive complex numbers (i.e. \code{24*sizeof(Float)} bytes where \code{Float} is a template parameter for real numbers (\code{double}, \code{float}, \code{half}) to or from the output array \code{v}. This is implemented in the order class \code{OpenQCDDiracOrder} in \code{include/color\_spinor\_field\_order.h} \cite{QUDApaper} and concludes spinor field reordering.

\subsubsection{Clover Field}

Similarly to the spinor field, for each space-time index, we can copy $72 = 2*36$ real numbers (i.e. \code{72*sizeof(Float)} bytes)
to the output array \code{v} (the save function is not necessary, since we never need to save clover fields from device to host).

openQxD stores the clover field as two arrays $u$ of length $36$ that represent two Hermitian 6$\times$ 6 matrices (one for each chirality $\pm$). The first $6$ entries are the diagonal real numbers and the following 15 pairs denote real and imaginary parts of the strictly upper triangular part in row-major order.
% \newlength{\oldcolsep}
% \setlength{\oldcolsep}{\arraycolsep}
% \setlength{\arraycolsep}{4pt}
% \begin{equation}{\small
% \begin{pmatrix}
% u_0   & u_6 + iu_7 & u_8 + iu_9       & u_{10} + iu_{11} & u_{12} + iu_{13} & u_{14} + iu_{15} \\
% \cdot & u_1        & u_{16} + iu_{17} & u_{18} + iu_{19} & u_{20} + iu_{21} & u_{22} + iu_{23} \\
% \cdot & \cdot      & u_2              & u_{24} + iu_{25} & u_{26} + iu_{27} & u_{28} + iu_{29} \\
% \cdot & \cdot      & \cdot            & u_3              & u_{30} + iu_{31} & u_{32} + iu_{33} \\
% \cdot & \cdot      & \cdot            & \cdot            & u_4              & u_{34} + iu_{35} \\
% \cdot & \cdot      & \cdot            & \cdot            & \cdot            & u_5
% \end{pmatrix}}\,.
% \end{equation}

% QUDA stores these 36 numbers in a similar format (see \code{include/clover\_field\_order.h} \cite{QUDApaper}):
% \begin{equation}{\small
% \begin{pmatrix}
% u_0              & \cdot            & \cdot            & \cdot            & \cdot            & \cdot \\
% u_6 + iu_7       & u_1              & \cdot            & \cdot            & \cdot            & \cdot \\
% u_8 + iu_9       & u_{16} + iu_{17} & u_2              & \cdot            & \cdot            & \cdot \\
% u_{10} + iu_{11} & u_{18} + iu_{19} & u_{24} + iu_{25} & u_3              & \cdot            & \cdot \\
% u_{12} + iu_{13} & u_{20} + iu_{21} & u_{26} + iu_{27} & u_{30} + iu_{31} & u_4              & \cdot \\
% u_{14} + iu_{15} & u_{22} + iu_{23} & u_{28} + iu_{29} & u_{32} + iu_{33} & u_{34} + iu_{35} & u_5
% \end{pmatrix}}\,. 
% \end{equation}
% \setlength{\arraycolsep}{\oldcolsep}

QUDA stores the strictly lower triangular part in column-major order. 
So we can transfer the clover field from openQxD to QUDA by specifying how these 36 numbers transform. In particular, the QED
clover field does not affect the block structure of the clover term and we can also transfer the clover term in QCD+QED (see \cref{sec:qcd+qed}
for details).
On the other hand, a pure QCD clover field can be calculated natively within QUDA and no additional transfer of fields is required in that case.

\subsubsection{Gauge Field}
    QUDA associates 4 gauge fields for each space-time point (one for each positive direction $\mu=0,1,2,3$), whereas openQxD stores $8$
    (forward and backward) directions of gauge fields for all odd-parity points (see \code{main/README.global} for more information \cite{openqxd}). When looking at local lattices in a multi-rank scenario, this implies that openQxD locally stores gauge fields on the boundaries only for odd-parity points and not for even-parity points (see \cref{fig:gauge}). These even-parity boundary fields are stored in a buffer space, but they have to be communicated from neighbouring lattices first.

\begin{figure}
  \centering
  \includestandalone[width=0.7\linewidth]{img/gauge} %without .tex extension
  % or use \input{mytikz}
  \caption{2D example ($4 \times 4$ local lattice) of how and which gauge fields are stored in memory in openQxD (left) and QUDA (right). Filled lattice points are even, unfilled odd lattice points. The red filled lattice point denotes the origin. Arrows represent gauge fields and the arrow head points to the lattice point where we store the field.}
  \label{fig:gauge}
\end{figure}

This requires us to transfer the missing gauge fields from one rank to the other before entering any QUDA interface function.
% The gauge field is loaded to and saved from QUDA by the following two API calls

% \begin{lstlisting}[language=C++]
% void loadGaugeQuda(void *h_gauge, QudaGaugeParam *param);
% void saveGaugeQuda(void *h_gauge, QudaGaugeParam *param);
% \end{lstlisting}

% where the void pointer \code{h\_gauge} points to the gauge fields in the CPU memory (the missing fields have to be available already) and \code{param} is a struct holding information about the gauge field and how it should be interpreted by the various Dirac operators supported by QUDA.

We implement an ordering class called \code{OpenQCDOrder} (see \code{include/gauge\_field\_order.h} \cite{QUDApaper}) with corresponding load and save methods. The only difference to the spinor and clover field order classes is that the methods are called with an additional direction variable \code{dir}. For a fixed space-time $x$ and direction, the remaining two color indices $(a,b)$ of the gauge field are row-major in both applications, thus we can copy $3\times 3$ consecutive complex numbers to or from \code{v}.

% \begin{lstlisting}[language=C++]
% __device__ __host__ inline void load(complex v[length/2], int x_cb, int dir, int parity, Float = 1.0) const
% __device__ __host__ inline void save(const complex v[length/2], int x_cb, int dir, int parity) const
% \end{lstlisting}

% The variable \code{dir} runs from $0$ to $3$ and denotes the positive link direction in QUDA convention (see \cref{fig:gauge} right).

\subsection{C\texorpdfstring{$^{\star}$}{*} boundary conditions}
\label{sub:cstar}

% Gauss's law prohibits dynamical simulations of charged particles in a finite box with periodic boundary conditions; $C^\star$ boundary conditions do not suffer from this restriction \cite{Kronfeld1991}.
% % , which are not yet implemented in QUDA. 
% The implementation of these conditions in QUDA is the focus of the current section.
% Unlike periodic boundary conditions, we identify the field shifted by one lattice length not with itself (periodic boundary conditions), but with
% its charge conjugation. A simple implementation consists in doubling the lattice size in $x$-direction (this choice of direction is arbitrary). We refer
%  to this as extended lattice, which consists of a physical and mirror lattice. The fields on the mirror lattice 
%  are related to the physical lattice by charge conjugation. Thus, C$^\star$ boundary conditions are implemented by translation from
%  physical to mirror lattice and choosing appropriate boundary conditions  (see \cref{fig:cstar}).

% \begin{figure}
%   \centering
%   \includestandalone[width=0.7\linewidth]{img/cstar}
%   \caption{2D example of a $6 \times 6$ lattice with C$^\star$ boundary conditions on both directions. We have the (doubled) x-direction (horizontal) and a direction with C$^\star$ boundaries (vertical). Left is the physical, right the mirror lattice. Unfilled lattice points are exterior boundary points, whereas filled points are interior (boundary) points. The points of the same color are identified with each other. Notice that in x-direction we have regular periodic boundary conditions, since C$^\star$ boundaries are periodic over twice the lattice extent. The red, green and blue arrows indicate the path
%   taken when leaving the physical lattice and entering the mirror lattice.}
%   \label{fig:cstar}
% \end{figure}

We choose to implement C$^\star$ boundary conditions in the same way as they are implemented in openQxD -- by doubling of the lattice in $x$-direction and by imposing shifted boundaries.
%as illustrated in \cref{fig:cstar}. Note that openQxD requires at least two ranks for C$^\star$ boundary conditions,
%which ensures that a rank stores points in either the physical or mirror lattice.

When QUDA initializes its communication grid topology, we specify the neighbours of each rank in all directions. The function \code{comm\_rank\_displaced()} in \code{include/communicator\_quda.h} \cite{QUDApaper} calculates the neighbouring rank number given one of (positive or negative) 8 directions. We change this function to achieve shifted boundary conditions
%as in \cref{fig:cstar}: Consider the case of two ranks, one of which contains all physical points, the other the mirror points. The neighbour of the physical lattice in "upward" direction is the mirror rank (and vice versa), which is different from periodic boundary conditions.

\subsection{QCD+QED}
\label{sec:qcd+qed}

% The Wilson-Clover Dirac operator in QCD simulations applied onto a spinor field $\psi(x)$ is (the lattice spacing is set to $a = 1$)
% \begin{equation}
% \begin{aligned} \label{eq:Dw}
% D_\mathrm{w} &\psi(x) = 4 \psi(x) \\
% -&\frac{1}{2} \sum_{\mu=0}^3 \Big\{
%   U_{\mu}(x) (1-\gamma_{\mu}) \psi(x + \hat{\mu})
% + U_{\mu}(x-\hat{\mu})^{-1} (1+\gamma_{\mu}) \psi(x-\hat{\mu})
% \Big\} \\
% +&c_\mathrm{sw}^{SU(3)} \frac{i}{4} \sum_{\mu,\nu=0}^3 \sigma_{\mu \nu} \hat{F}_{\mu \nu}(x) \psi(x),
% \end{aligned}
% \end{equation}
% where the gauge field $U_{\mu}(x)$ is the $SU(3)$-valued link between lattice point $x$ and $x + \hat{\mu}$, the $\gamma_{\mu}$ are the Dirac matrices obeying the Euclidean Clifford algebra, $\{\gamma_{\mu}, \gamma_{\nu}\} = 2 \delta_{\mu \nu}$ and $\sigma_{\mu \nu} = \frac{i}{2} \left[\gamma_{\mu}, \gamma_{\nu}\right]$. The last term is called SW-term (or clover term) and is block-diagonal. The $SU(3)$ field strength tensor $\hat{F}$ is defined as

% \begin{align*}
% \hat{F}_{\mu \nu}(x) &= \frac{1}{8} \left\{
%     Q_{\mu \nu}(x) - Q_{\nu \mu}(x)
% \right\}, \\
% Q_{\mu \nu}(x)
% &= U_{\mu}(x)
%    U_{\nu}(x+\hat{\mu})
%    U_{\mu}(x+\hat{\nu})^{-1}
%    U_{\nu}(x)^{-1} \\
% &+ U_{\nu}(x)
%    U_{\mu}(x-\hat{\mu}+\hat{\nu})^{-1}
%    U_{\nu}(x-\hat{\mu})^{-1}
%    U_{\mu}(x-\hat{\mu}) \\
% &+ U_{\mu}(x-\hat{\mu})^{-1}
%    U_{\nu}(x-\hat{\mu}-\hat{\nu})^{-1}
%    U_{\mu}(x-\hat{\mu}-\hat{\nu})
%    U_{\nu}(x-\hat{\nu}) \\
% &+ U_{\nu}(x-\hat{\nu})^{-1}
%    U_{\mu}(x-\hat{\nu})
%    U_{\nu}(x+\hat{\mu}-\hat{\nu})
%    U_{\mu}(x)^{-1}.
% \end{align*}

In QCD+QED simulations, in addition to the $SU(3)$-valued gauge field $U_\mu(x)$, we have the $U(1)$-valued gauge field $A_\mu(x)$, which when combined results
in a $U(3)$-valued field $e^{i q A_\mu(x)} U_\mu(x)$ with $q_f$ the charge of a quark. These links are produced by multiplying the $U(1)$ phase to the $SU(3)$ matrices, which can be done in openQxD. For a QCD+QED operator in QUDA, we just upload these $U(3)$-valued links instead of the $SU(3)$ ones.

% In addition, we add another SW-term,
% \begin{equation} \label{eq:Dw2}
% D_\mathrm{w} \rightarrow D_\mathrm{w} + q c_\mathrm{sw}^{U(1)} \frac{i}{4} \sum_{\mu,\nu=0}^3 \sigma_{\mu \nu} \hat{A}_{\mu \nu}\,,
% \end{equation}
% where $q$ is the charge and the $U(1)$ field strength tensor $\hat{A}_{\mu \nu}(x)$ is defined as
% \begin{align*}
% \hat{A}_{\mu \nu}(x) &= \frac{i}{4 q_{el}} \text{Im} \left\{
%       z_{\mu \nu}(x)
%     + z_{\mu \nu}(x-\hat{\mu})
%     \right. \\
%     &\phantom{=\frac{i}{4 q_{\text{el}}} \text{Im} \left\{ \right.} \left. 
%     + z_{\mu \nu}(x-\hat{\nu})
%     + z_{\mu \nu}(x-\hat{\mu}-\hat{\nu})
% \right\} \\
% z_{\mu \nu}(x) &= e^{i\left\{
%       A_{\mu}(x)
%     + A_{\nu}(x+\hat{\mu})
%     - A_{\mu}(x+\hat{\nu})
%     - A_{\nu}(x)
% \right\}}
% \end{align*}

In addition, we add another SW-term proportional to its coefficient $c_{SW}^{U(1)}$. Therefore, the QCD+QED Clover term consists of both the $SU(3)$ and the $U(1)$ term, which can be calculated in openQxD. The resulting term is still diagonal in space-time and chirality, and is Hermitian in color and spin. Therefore it has the same representation in memory as the $SU(3)$ clover term alone and we can just upload this new clover field to QUDA using the clover field reordering class that we have already implemented.

Transferring the QCD+QED clover term, the $U(3)$ links as well as the changes in the process grid topology enables QUDA to handle the QCD+QED Wilson-Clover Dirac operator. This concludes our first implementation of QCD+QED in QUDA.

% \end{document}


==> __sections/05-solver.tex <==
% This allows for compiling the file separately:
% \documentclass[main.tex]{subfiles}

% \begin{document}

% A main program in openQxD that wants to leverage QUDAs solvers may be changed in the following way.
In order to use QUDA in openQxD, we 
 include the necessary header files that provide the interface to QUDA, and link it with the compiled QUDA library (details on linking the library are discussed in \cref{building_openqxd_against_quda}):

\begin{lstlisting}[language=C++]
#include "quda_utils.h"
#include <quda_openqcd_interface.h>
\end{lstlisting}

In this example \code{quda\_utils.h} is a header file in openQxD that provides the function
\begin{lstlisting}[language=C++]
openQCD_QudaInitArgs_t quda_init(void);
\end{lstlisting}
This function takes no arguments and its return struct can be ignored (it is used in some of the tests). The function initializes a struct that describes the lattice setup such as boundary conditions (return value of \code{bc\_parms()}), Dirac parameters (return value of \code{dirac\_parms()}), gauge group (\code{flds\_parms()}), local lattice dimensions, process grid and its mapping to MPI ranks, process block grid, pointers to the gauge and clover fields. All these structs have to be set before calling \code{quda\_init()}. This information is passed to QUDA by calling \code{openQCD\_qudaInit()} in \code{quda\_openqcd\_interface.h}, which itself initializes the communication grid (and arranges the ranks as needed by the boundary conditions). QUDA is then initialized by calling \code{initQuda()}.

The header file \code{quda\_openqcd\_interface.h} provides API functions to set up, invoke and destroy the solver context \footnote{Notice that these function names might be subject of change in the near future.}.

\begin{lstlisting}[language=C++]
void* openQCD_qudaSolverSetup(char *infile,
                              char *section);
double openQCD_qudaInvert(void *param, double mu,
                          void *source, void *solution,
                          int *status);
void openQCD_qudaSolverDestroy(void *param);
\end{lstlisting}

The function \code{openQCD\_qudaSolverSetup()} takes two parameters; a path to an input file and a section name. The input file looks like a regular openQCD input file in a dialect of the INI file format. This input file is assumed to have a section given by the section name, where the QUDA-solver is described:

\begin{lstlisting}[]
[Solver ABC]
solver          QUDA
maxiter         2048
gcrNkrylov      20
tol             1e-4
reliable_delta  1e-5
inv_type        QUDA_GCR_INVERTER
verbosity       QUDA_VERBOSE
\end{lstlisting}

The section name in the above example is \code{Solver ABC}. For the section to be a valid QUDA-solver section we need the key-value pair \code{solver = QUDA} in the section, else the setup function will throw an error message. All the remaining keys parameterize the various members of the struct \code{QudaInvertParam} and we refer the reader to its documentation (see \code{Wiki} on \cite{QUDApaper}). The example section above is minimal, i.e. it only sets required parameters; it solves the Wilson-Clover Dirac equation using a GCR solver without any preconditioning to a residual of $\text{tol} = $\code{1e-4}. The setup function \code{openQCD\_qudaSolverSetup()} returns a void pointer that acts as a solver handle holding all the relevant information.

When calling the solver with \code{openQCD\_qudaInvert}, the function expects this solver handle as its first parameter. In order to mimic the behaviour of the openQCD solvers (e.g. \code{tmcg}, \code{sap\_gcr}, \code{dfl\_sap\_gcr}), the invert-function accepts a twisted mass parameter \code{mu} explicitly. The two following parameters are the \code{source} and \code{solution} vectors given as regular openQCD arrays of \code{spinor\_dble} that might have been allocated and reserved using \code{alloc\_wsd()} and \code{reserve\_wsd()} respectively. Note that both spinor fields, \code{source} and \code{solution}, have to be allocated on the CPU and \code{source} might be initialized as a point or random source at this point. Finally the \code{status} variable is set to a negative integer if the solver fails and to a positive number (number of outer iteration steps) otherwise.

When the solver is not needed anymore, the data structs can be deallocated by calling the destroy function \code{openQCD\_qudaSolverDestroy()}, which also takes the solver handle as its only argument.

Finally, to destroy the QUDA context entirely, we call the finalize function:

\begin{lstlisting}[language=C++]
void openQCD_qudaFinalize(void);
\end{lstlisting}

This interface makes all variants of the iterative solver algorithms in the QUDA library for Wilson fermions accessible in openQxD, including the conjugate gradient (CG), generalized conjugate residuals (GCR) and the adaptive multi-grid preconditioner (MG)~\cite{Babich:2010qb} which is similar to the inexact deflation method implemented natively in openQxD. 
% \end{document}

==> __sections/06-building.tex <==
% This allows for compiling the file separately:
% \documentclass[main.tex]{subfiles}

% \begin{document}

% \subsection{Environment setup and recommended versions}







% Compiling QUDA and openQxD each require to have some environment variables declared to correctly compile them and make use of their features, we refer to the documentations for their independent compilation's details.

% Compiling QUDA and openQxD requires the declaration of certain environment variables. Detailed instructions for these independent compilation processes can be found in their respective documentation.

% Regarding compiling the OpenQxD for 

% , it's important to note that OpenQxD assumes the environment variables \code{GCC}, \code{MPI\_HOME}, and \code{MPI\_INCLUDE} are set to the path to the gcc compiler, the MPI installation directory, and the path to the directory where \code{mpi.h} is located. The compilation of OpenQxD programs for interfacing with QUDA is performed by using the C99 standard instead of C89, which is the one present in the official OpenQxD release v.1.1.



A recommended compilation from scratch is presented below, first by compiling the QUDA library according to our simulation's needs, then by compiling openQxD with the QUDA library linked to it.

\subsection{QUDA}

QUDA needs to be compiled as a library. We refer to the QUDA documentation \cite{QUDApaper} for generic compilation instructions and focus
on enabling support for openQxD.

%To build QUDA v.1.1.0 (develop), we need an installation of CMake v.3.18 or later. For compiling QUDA, an installation of the CUDA toolkit v.11.0 at least is recommended\footnote{ref:QUDA documentation}, as well as compilers that have support for the C++17 standard, such as gcc v.5.0 or later for partial support, or gcc v.9.0 or later for full C++17 support. Alternatively, QUDA can be compiled with the C++14 by setting CMake accordingly.

%When compiling QUDA with MPI, we require an MPI implementation adopting the 4.0 standard at least.

% Regarding support for the C++17 standard\todo{add ref:}\footnote{ref:https://gcc.gnu.org/projects/cxx-status.html}, which is used throughout QUDA, we require at least gcc v.9 for full support of its features, (in our system we use gcc v.11.4). Finally, for MPI support, QUDA developers recommend at least OpenMPI v.4.0.x (we use OpenMPI v.4.1.2).

%For details of how to setup environment variables for a successful QUDA compilation, we refer to CMake \todo{rm:v.3.18} documentation \todo{add ref}.

% When CMake builds QUDA, it will detect environment variables essential for QUDA's compilation. In case some variables are not defined, CMake will try and define them according to your system, but this could not properly work in a given system, and it is thus recommended to declare some of them from start. For example, in our system environment, we defined the following.

% \begin{lstlisting}[language=bash]
% # GCC compilers, make sure it is gcc version 9.x at least
% export CC=/usr/bin/x86_64-linux-gnu-gcc-11
% export GCC=${CC}
% export CXX=/usr/bin/x86_64-linux-gnu-g++-11
% export CF=/usr/bin/x86_64-linux-gnu-gfortran-11

% # MPI support, make sure it is OpenMPI version 4.0.x at least
% export MPI_HOME=/usr/lib/x86_64-linux-gnu/openmpi
% export MPI_INCLUDE=${MPI_HOME}/include
% # Add MPI to libpath
% export LD_LIBRARY_PATH=${MPI_HOME}/lib:${LD_LIBRARY_PATH}

% # CUDA Toolkit and compilers, make sure it is v.11.0 at least
% export CUDA_HOME=/usr/local/cuda-11.6
% export CUDACXX=/usr/local/cuda-11.6/bin/nvcc
% export CUDA_BIN_PATH=/usr/local/cuda-11.6/bin
% # Add CUDA_BIN to PATH
% export PATH=${CUDA_BIN_PATH}$:${PATH}
% \end{lstlisting}

Building QUDA with support for the openQxD interface requires setting a few CMake build-flags. To enable the Wilson-Clover Dirac operator we set the following flags in \code{CMakeLists.txt} \cite{QUDApaper}:
\begin{lstlisting}[]
QUDA_DIRAC_DEFAULT_OFF=ON # disables ALL Dirac operators
QUDA_DIRAC_WILSON=ON      # enables Wilson-Dirac
                          # operators
QUDA_DIRAC_CLOVER=ON      # enables Wilson-clover
                          # operators
\end{lstlisting}
We enable the openQCD interface by setting
\begin{lstlisting}[]
QUDA_INTERFACE_OPENQCD=ON # enable openQCD interface
QUDA_RECONSTRUCT=4        # no gauge field reconstruction
\end{lstlisting}
(the gauge fields in openQxD are not compressed so we do not need to reconstruct them). Furthermore we enable multi-GPU support and the multigrid solver by
\begin{lstlisting}[]
QUDA_MPI=ON          # enable MPI
QUDA_MULTIGRID=ON    # enable multigrid solvers
\end{lstlisting}

\subsection{openQxD}

After QUDA is built according to the previous section, we compile openQxD. Note that we require a compiler compliant with the C89 and the MPI 1.2 standard. We refer the user to the official openQxD documentation \cite{openqxd} on how to compile and focus here on the changes that have to be made to compile against QUDA. Note that we need to dynamically link every openQxD binary that wants to use the QUDA library.

% ref: https://gitlab.com/rcstar/openQxD README
% \todo{add ref to OpenQxD docs on compiling}, with the exception of needing to 

Hence, when compiling an openQxD program, we add the path to QUDA's \code{include} directory (e.g., \code{-I<path>} for gcc), the path to QUDA's \code{lib} directory (e.g., \code{-L<path>} for gcc), and the named library (e.g., \code{-lquda} for gcc) in the linking phase. An example \code{Makefile} can be found under \code{devel/quda/Makefile} in the openQxD repository \cite{openqxd}.

% Note that any modification to the lattice geometry in OpenQxD (i.e., in \code{global.h}) necessitates recompiling the program binaries. 

% For the dynamic linking of OpenQxD:
% \code{
% export LD_LIBRARY_PATH=/scratch/jfernande/quda_openqxd/openqxd_quda_build/build/lib:\${LD_LIBRARY_PATH}
% }


% \end{document}


==> __sections/07-performance.tex <==
% This allows for compiling the file separately:
% \documentclass[main.tex]{subfiles}

% \begin{document}
To obtain preliminary indications of the performance of the QUDA library on GPUs on the typical problem sizes and parameters relevant to our physics programme. For the comparison of the inversions between CPU and GPU implementations, we note that the multi-grid algorithm implemented in QUDA is not exactly the inexact deflation available in openQxD, therefore we anticipate further optimization of its parameters will improve its performance in future.

\begin{table}[h]
\centering
\begin{tabular}{ccccc}
Name & Global size $V_\mathrm{G}$ & Pion mass & Boundary conditions \\
\hline
G8   & $64^3 \times 128$ & $180$ MeV & periodic \\
C380 & $48^3 \times 96$  & $380$ MeV & C$^\star$ \\
\end{tabular}
\caption{The lattice ensembles used for the performance tests of the inversion of the Dirac operator. G8 has been generated by the CLS initiative~\cite{cls}, while C380 is generated by the RC$^\star$ collaboration~\cite{RCstar22}. The last column refers to spatial boundary conditions.}
\label{tab:ensembles}
\end{table}

% \subsection{Hardware specifications}
% \label{sec:hardware}

% The performance measures that follow are obtained on the machines
% \begin{itemize}
%     \item Piz Daint multicore at CSCS, Switzerland, 2x Intel® Xeon® E5-2695 v4 @ 2.10GHz (2x 18 cores, 64/128 GB RAM)
%     \item Piz Daint hybrid at CSCS, Switzerland, 1x Intel® Xeon® E5-2690 v3 @ 2.60GHz (12 cores, 64GB RAM) and 1x NVIDIA® Tesla® P100 16GB
%     \item LUMI-C at CSC, Finland, 2x AMD EPYC 7763 @2.45GHz (2x 64 cores, 256-1024 GB RAM)
%     \item LUMI-G at CSC, Finland, 1x AMD® Trento™ (64 cores, 512 GB RAM) and 4x AMD® Instinct™ MI250X GPU 128GB
% \end{itemize}

% \subsection{Dirac operator}

% We investigate the scaling behaviour of applying the Dirac stencil operator, \cref{eq:Dw,eq:Dw2}, both in openQxD as well as  QUDA, see \cref{fig:daint_dw_strong,fig:daint_dw_weak,fig:lumi_dw_strong,fig:lumi_dw_weak}. We see very good strong and weak scaling on the CPU. Notice that the base case of the GPU version is one GPU (i.e. no network communication) for the periodic lattice and 8 GPUs for the C$^\star$ lattice \footnote{The current implementation demands a process grid length of at least 2 in every direction that is a spatial C$^\star$-direction. With 3 C$^\star$ directions this gives a minimum of 8 processes, i.e. 8 GPUs.}. We use 32 and 128 ranks per node in the CPU runs for Piz Daint and LUMI-C, respectively. The GPU runs are limited by network communication more severely than the CPU runs. For the weak scaling plots we make sure that node- and GPU-local lattices have the same size. The strong and weak scaling seems less favourable on the GPU, but when comparing the time to solution, we see a $\sim10$x speedup between CPU and GPU runs for the same problem size and moderate amounts of GPUs. In \cref{fig:daint_dw_weak} right, we observe the (expected) $\sim2$x slowdown of a C$^\star$ operator compared to a periodic one on the same device and setup, due to a doubling of the lattice size in $x$-direction.

% The poor scaling of the application of the Dirac operator on LUMI-G (\cref{fig:lumi_dw_strong,fig:lumi_dw_weak}) can probably be explained by the high computational performance of the MI250 which exposes us to the limited communication bandwidth earlier. To make best use of resources a larger local volume would be favourable to keep the device utilized while reducing the communication overhead (due to a smaller surface-to-volume ratio). In our tests, we use the same lattice size on Piz Daint as well as on LUMI-G to be able to compare them, and the P100 with 16GB DRAM on Piz Daint was the limiting factor. However, this suggests that the way we've implemented C$^\star$ boundaries (namely by doubling the lattice) is favourable for the GPU, because it makes the local lattice larger.

% \begin{table*}
% \begin{tabular}{l|ll|ll}
% \toprule
%  & \multicolumn{4}{c}{cost in node-seconds [sec]} \\
% \midrule
%  & \multicolumn{2}{c}{periodic ($V_\mathrm{G}=64\times32\times32\times64$)} & \multicolumn{2}{c}{C$^\star$ ($V_\mathrm{G}=128\times64\times64\times64$)} \\
% \midrule
% nodes/GPUs & Piz Daint GPU & Piz Daint CPU & Piz Daint GPU & Piz Daint CPU \\
% \midrule
%    1 & 0.023146040(628) &  0.162241(174) &              &  1.2444(117) \\
%    2 &    0.023661(178) &  0.163499(376) &              & 1.24068(475) \\
%    4 &    0.025835(708) &   0.17126(101) &              & 1.32666(613) \\
%    8 &    0.042252(302) &  0.174588(889) & 0.23470(762) &  1.3596(146) \\
%   16 &     0.06203(113) &   0.18817(131) & 0.31696(994) & 1.44997(168) \\
%   32 &     0.07759(142) &   0.18814(254) & 0.40192(427) &  1.5171(143) \\
%   64 &     0.09055(397) &   0.20222(196) & 0.47902(636) &  1.5349(228) \\
%  128 &    0.111636(701) &   0.26917(683) & 0.58217(911) &  1.6314(153) \\
%  256 &     0.22056(302) &   0.34688(534) &  0.6954(230) &  1.8859(191) \\
%  512 &     0.35585(533) & 0.434372608(0) &  0.9402(558) &  2.0787(331) \\
% 1024 &       0.667(141) &                &  1.2964(951) &              \\
% \bottomrule
% \end{tabular}
% \caption{Cost in node-seconds of one application of the Dirac operator on Piz Daint (see \cref{sec:hardware}). The global lattices are held constant.}
% \label{tab:nodehours_daint}
% \end{table*}

% \begin{table*}
% \begin{tabular}{ll|ll|ll}
% \toprule
%  && \multicolumn{4}{c}{cost in node-seconds [sec]} \\
% \midrule
%  && \multicolumn{2}{c}{periodic ($V_\mathrm{G}=64\times32\times32\times64$)} & \multicolumn{2}{c}{C$^\star$ ($V_\mathrm{G}=128\times64\times64\times64)$} \\
% \midrule
% nodes & GPUs & LUMI GPU & LUMI CPU & LUMI GPU & LUMI CPU \\
% \midrule
%   1 &    1 & 0.015923220(595) &               &              &              \\
%   1 &    2 &   0.0077102(141) &               &              &              \\
%   1 &    4 &    0.005683(714) &               &              &              \\
%   1 &    8 &    0.005751(579) & 0.044532(772) & 0.03834(325) & 0.34713(141) \\
%   2 &   16 &    0.008744(472) & 0.045384(362) & 0.04359(476) & 0.35914(313) \\
%   4 &   32 &     0.01111(239) &  0.04758(468) &  0.0635(125) & 0.37067(156) \\
%   8 &   64 &     0.01123(100) & 0.047173(458) &  0.0724(160) & 0.40354(185) \\
%  16 &  128 &     0.01679(148) &  0.04909(394) &  0.0726(118) & 0.40973(421) \\
%  32 &  256 &     0.02214(183) & 0.047487(869) &  0.0926(169) & 0.40900(786) \\
%  64 &  512 &     0.03478(155) & 0.052639(898) &  0.1212(206) &   0.538(118) \\
% 128 & 1024 &     0.05901(380) &  0.06068(222) &  0.1654(113) &              \\
% \bottomrule
% \end{tabular}
% \caption{Cost in node-seconds of one application of the Dirac operator on LUMI-G and LUMI-C (see \cref{sec:hardware}).  The global lattices are held constant. Notice that we count $8$ GPUs per node on LUMI-G, since one AMD MI250 abstracts itself as $2$ GPUs from the point of view of the program.}
% \label{tab:nodehours_lumi}
% \end{table*}

% In conclusion, we see a speedup for the time to solution, even if the strong and weak scaling seem poor for the GPU runs. However, we expect better scaling for larger problem sizes with a small surface to volume ratio.

% Finally, looking at the cost in terms of node-hours, \cref{tab:nodehours_daint,tab:nodehours_lumi}, we see that the GPU runs are cheaper by nearly an order of magnitude. LUMI-G is a clear winner here. % that's the only case where lumi wins ...
% When comparing the cost of periodic and C$^\star$, notice that the physical lattice for the C$^\star$ runs is $4$x larger than the periodic one: a factor of $4$ is thus expected.

% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{img/daint_dw_strong}
%     \caption{Strong scaling (left) and time for one application (right) of the Dirac operator on Piz Daint (see \cref{sec:hardware}) on the CPU (circles) and GPU (crosses) using a periodic (red) and a lattice with 3 C$^\star$ directions (blue). The x-axis denotes the number of nodes for CPU runs (32 ranks per node) and number of GPUs for GPU runs (1 P100 GPU per node). The global lattice sizes are $V_\mathrm{G} = (64 \times 32 \times 32 \times 64)$ and $V_\mathrm{G} = (64 \times 64 \times 64 \times 128)$ for the periodic and C$^\star$ runs, respectively.}
%     \label{fig:daint_dw_strong}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{img/daint_dw_weak}
%     \caption{Weak scaling (left) and time for one application (right) of the Dirac operator on Piz Daint (see \cref{sec:hardware}), the setup is the same as in \cref{fig:daint_dw_strong}. The node- or GPU-local lattice sizes are $V_\mathrm{L} = (32 \times 32 \times 32 \times 32)$ and $V_\mathrm{L}= (64 \times 32 \times 32 \times 32)$ for the periodic and C$^\star$ runs, respectively. Notice that the physical lattice is of the same size in both cases (the C$^\star$ lattice needs to be doubled in one of the spatial directions).}
%     \label{fig:daint_dw_weak}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{img/lumi_dw_strong}
%     \caption{Strong scaling (left) and time for one application (right) of the Dirac operator on LUMI-G and LUMI-C (see \cref{sec:hardware}). Notice that for the x-axis, number of GPUs is not the same as the number of nodes. A LUMI-G nodes has 4x AMD MI250s, logically abstracted as 8 GPUs.}
%     \label{fig:lumi_dw_strong}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{img/lumi_dw_weak}
%     \caption{Weak scaling (left) and time for one application (right) of the Dirac operator on LUMI-G (see \cref{sec:hardware}).}
%     \label{fig:lumi_dw_weak}
% \end{figure}

\subsection{Solving the Dirac equation}

For solving the Dirac equation, we use a heavily preconditioned GCR algorithm. In case of the CPU runs, we use openQxD's deflated mixed-precision%
\footnote{single and double precision IEEE-754 floats} GCR solver that uses Schwarz alternating procedure as a preconditioner (\code{DFL\_SAP\_GCR} in openQCD parlance). The GPU runs use QUDAs mixed-precision%
\footnote{half, single and double precision IEEE-754 floats} multi-grid GCR solver (MG). The two solvers are very similar in how they generate the coarse grid subspace. The CPU solver parameters are tuned, but due to lack of experience with multi-grid, we used a somewhat not optimised parameter set for multi-grid on the GPU. The relative residual is chosen to be $10^{-12}$ for all solves.

We obtain good weak scaling, see \cref{fig:inv_weak}. Again, LUMI outperforms Piz Daint in terms of cost. This is expected, since one LUMI-G node contains $4$ AMD MI250s (abstracted as $8$ devices) and one Piz Daint hybrid node contains a single NVIDIA P100. The factor is not 4x, but rather $\ge10$x, which is explained by the higher memory bandwidth of the former GPU \footnote{P100: 720 GB/s \cite{nv_p100} vs. MI250: 3.2768 TB/s \cite{amd_mi250}.}.
We note that strong-scaling for multi-grid algorithms is inherently challenging due to the reduced numbers of degrees of freedom on the coarser levels, which requires new algorithmic ideas~\cite{Espinoza-Valverde:2022pci}.

% \begin{table}
% \begin{tabular}{l|l|l}
% \toprule
%  & \multicolumn{2}{c}{cost in node-seconds [sec]} \\
% \midrule
% GPUs & LUMI-G & Piz Daint \\
% \midrule
%  32 & 34.6 &  347 \\
%  64 & 70.0 &  748 \\
% 128 & 159  & 1693 \\
% 256 & 349  & 3584 \\
% 512 & 825  & 8558 \\
% \bottomrule
% \end{tabular}
% \caption{Cost in node-seconds of one solve of the Dirac equation. The GPU-local lattice is held constant ($V_\mathrm{L}=32x32x32x32$).}
% \label{tab:nodehours_inv}
% \end{table}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{img/inv_weak}
    \caption{Weak scaling (left) and time to solution (right) for one solve of the Dirac equation on LUMI (blue) and on Piz Daint (red) on the CPU (circle) and GPU (crosses) partition. Runs were conducted on machines: Piz Daint multicore at CSCS, Switzerland, 2x Intel® Xeon® E5-2695 v4 @ 2.10GHz (2x 18 cores, 64/128 GB RAM),
    Piz Daint hybrid at CSCS, Switzerland, 1x Intel® Xeon® E5-2690 v3 @ 2.60GHz (12 cores, 64GB RAM) and 1x NVIDIA® Tesla® P100 16GB,
    LUMI-C at CSC, Finland, 2x AMD EPYC 7763 @2.45GHz (2x 64 cores, 256-1024 GB RAM),
    and LUMI-G at CSC, Finland, 1x AMD® Trento™ (64 cores, 512 GB RAM) and 4x AMD® Instinct™ MI250X GPU 128GB.}
    \label{fig:inv_weak}
\end{figure}

% \end{document}


==> __sections/08-outlook.tex <==
% This allows for compiling the file separately:
% \documentclass[main.tex]{subfiles}

% \begin{document}

In summary, we are able to use GPUs efficiently to solve the Dirac equation for a sample background gauge configuration from the Markov chain through our interface to the QUDA library.
The good performance observed with the QUDA multi-grid algorithm will allow us to perform efficient operations which underpin the measurement part of the workflow for fixed background gauge field and reduce the statistical and systematic precision on our lattice QCD predictions.
We plan to further develop and optimize this part (see  \cref{sec:optimizations}).

As a continuation of this project, we aim to port the generation of gauge configurations to GPUs. This will involve updating the gauge and clover field regularly, since these change periodically during the Markov chain. To solve this problem, and mitigate unnecessary transfer of fields from host to device, we design a powerful memory management system.

\subsection{Optimizations}
\label{sec:optimizations}

We plan to run simulations on Alps, the successor of Piz Daint at CSCS. This machine will have NVIDIA H100 GPUs. Unlike P100 GPUs, the H100 support NVSHMEM - a technology for inter-node communication in a multi-GPU scenario. Documentation claims excellent strong scaling of up to 1000 GPUs \cite{nvshmem}. QUDA supports this communication layer already and no new implementation effort has to be done to profit from it.

For the generation of gauge ensembles the gauge field changes frequently which will trigger recurring host-to-device (H2D) transfers of the field. To reduce CPU-GPU communication for QCD+QED simulations, we want to avoid a recomputation of the clover field on the CPU and a subsequent H2D transfer. We plan to implement the generation of the clover field on the GPU directly in QUDA.

In a second stage, we plan to unify the spinor fields among the two applications. The key idea is to not deal with fields on the CPU separately from fields on the GPU. A challenge is that the two applications have a vastly different memory layouts for fields and reordering has to be performed from one to the other. In openQxD a spinor field is just a large array of structs, whereas in QUDA a field is a C++ object. We plan to implement a memory management system, that keeps track the field status and implicitly transfer the field only if required.

% \end{document}

